Towards a Neural Graphics Pipeline for Controllable Image Generation

In this paper, we leverage advances in neural networks towards forming a neural rendering for controllable image generation, and thereby bypassing the need for detailed modeling in conventional graphics pipeline. To this end, we present Neural Graphics Pipeline (NGP), a hybrid generative model that brings together neural and traditional image formation models. NGP decomposes the image into a set of interpretable appearance feature maps, uncovering direct control handles for controllable image generation. To form an image, NGP generates coarse 3D models that are fed into neural rendering modules to produce view-specific interpretable 2D maps, which are then composited into the final output image using a traditional image formation model. Our approach offers control over image generation by providing direct handles controlling illumination and camera parameters, in addition to control over shape and appearance variations. The key challenge is to learn these controls through unsupervised training that links generated coarse 3D models with unpaired real images via neural and traditional (e.g., Blinn- Phong) rendering functions, without establishing an explicit correspondence between them. We demonstrate the effectiveness of our approach on controllable image generation of single-object scenes. We evaluate our hybrid modeling framework, compare with neural-only generation methods (namely, DCGAN, LSGAN, WGAN-GP, VON, and SRNs), report improvement in FID scores against real images, and demonstrate that NGP supports direct controls common in traditional forward rendering. Code is available at http://geometry.cs.ucl.ac.uk/projects/2021/ngp.

==> fid_table.tex <==


\begin{table}[h!]
    \centering
    \caption{FID score, lower is better,  comparison on composition images data. All baseline methods are trained on composite images. \todo{to be deleted}}
      \begin{tabular}{c|ccccc}
            & DCGAN & LSGAN & WGAN-GP & VON   & Ours \\
      \midrule \midrule
      car   & 126.8 & 257.9 & 160.3 & 120.6 & \textbf{35.4} \\
      \midrule
      chair & 142.2 & 162.9 & 126.6 & 64.8  & \textbf{31.1} 
      \end{tabular}%
    \label{tab:fid_table}%
  \end{table}%


==> fid_table_real.tex <==
\begin{table}[b!]
    \begin{minipage}{.5\linewidth}
    \centering
    \tiny
    \caption{FID comparison on real images data. Note that FIDs are computed against real images data.}
      
      \begin{tabular}{r|ccccccc}
        \toprule
            & DCGAN & LSGAN & WGAN-GP & VON  & \oursbp  & \ours \\
          \midrule
          car   &130.5 & 171.4 & 123.4 & 83.3 & \textbf{67.2} & \textbf{58.3} \\
          \midrule
          chair & 225.0 & 225.3 & 184.9 & 51.8 & \textbf{47.9} & \textbf{51.2}  \\
         \bottomrule
        \end{tabular}%
    \label{tab:fid_table_onreal}
    \end{minipage}\hfill
    \begin{minipage}{.45\linewidth}
    \centering
    \tiny
    \caption{SRNs comparison. Note FIDs are computed against Blinn-Phong images data.}
      
      \begin{tabular}{r|cc}
        \toprule
              & SRNs  & \oursbp \\
        \midrule
        car   & 167.0 & \textbf{30.0} \\
        \midrule
        chair & 50.3  & \textbf{32.0} \\
        \bottomrule
      \end{tabular}%
    \label{tab:fid_table_srns}
    \end{minipage}\hfill
\end{table}

==> todelete_intro.tex <==
\section{Introduction}

For image generation,  we first model a scene with complete geometric details, and then generate realistic images by forward rendering the scene. 
Setting up such scenes in traditional computer graphics involves specifying object-level geometry and materials, along with providing camera and illumination parameters. 
Such images replace the need for physical photo-shoot, and hence are being adapted for creating product images, architectural previews, marketing catalogs, etc.
The main advantage of such a workflow is \textit{controllability} in the form of updating the scene geometry and materials, along with freely changing camera and illumination. 
The main bottleneck is to explicitly having to author complete and detailed scene geometry and materials specifications. 


An alternate approach is to directly create realistic images using an end-to-end  generative model. 
Advances in machine learning, particularly generative adversarial networks~(GANs), have revolutionized such a workflow. 
These methods attempt to match the distribution of high-dimensional features of the generated content with those of the training images, and thus prevent a discriminator, and also humans, from telling apart real and synthesized images. 
However, current GANs, either in 2D~\cite{xx} or in 3D~\cite{xx}, offer limited controls to the user. 
While it is possible to provide guidance through style example~\cite{gatys2016imagestyletransfer} or semantic specifications~\cite{spade}, it is often difficult to directly control 
generated imagery by updating geometry, camera, illumination, or material parameters. This lack of classical controls, supported by a traditional modeling paradigm, hinders  easy adaptation of these image generation workflows. 


In this work, we introduce {\em neural modeling} that produces coarse 3D content, decorated with view-specific interpretable 2D features, that can then be handled using traditional forward rendering approaches. 
The key observation is that the end-goal of many content creation applications is high-quality controllable image generation, and the input scene specification is only a proxy to enable this. 
Hence, we directly realize the above goal as coarse geometry generation followed by interpretable feature learning scaffolded off the coarse geometry, such that the hybrid representation can be used to produce high quality images. 
This has two main advantages: first, the synthesized geometric scaffold is coarse and does not need to be produced in full geometric details; and 
second, our representation is rendered using established rendering models (we use Blinn-Phong) and hence supports traditional camera and illumination changes. 
Thus, in contrast to traditional modeling paradigm that produces high-quality geometry and materials, our neural modeling produces coarse geometry with interpretable features. When rendered using popular rendering models, both representations produce high-quality images and are similarly controllable. 

Realizing the above goal requires overcoming multiple challenges. First, we do not have direct supervision data for the interpretable features. Second, we do not have access to high-quality models (i.e., geometry and material) in sufficiently large volumes. We either have a handful of high-quality models carefully created by skilled artists, or larger volumes of publicly available low to medium quality 3D model collections. 
Finally, while we can get access to large volumes of high-quality images, they come without correspondence to underlying 3D scenes, or camera and illumination information.  


We design neural modeling (see figure \ref{fig:neural modeling}), which consist of: (i)~generating coarse geometry using a 3D GAN;  (ii)~projecting the coarse scaffold using camera parameters to get 2D image-space mapping; and (iii)~learning a set of interpretable 2D reflectance features (i.e., normal, diffuse) that can be controlled and rendered under target illumination to produce final images. 
Such a design allows to handle the challenges described earlier. 
First, we use an unsupervised learning setup for the proposed framework. 
Second, we use low-quality 3D models (i.e., geometry and/or materials) to train a generative network to produce coarse 3D geometry and link them to 2D images via a known rendering function to learn interpretable intermediate features. 
Finally, by generating intermediate reflectance maps, we link the 3D and 2D datasources without requiring explicit correspondence information to utilize the heterogeneous sources of data. 



We extensively evaluate our neural modeling framework against several competing GAN-based image generation approaches and rate the different methods using a combination of established metrics. Our tests demonstrate the superiority of our method compare to other sate-of-the-art alternatives. \dc{What about the control aspect?? also I know there are deep methods that rendering 3D scenes represented in latent space}





\begin{figure}[b]
    \centering
	\includegraphics[width=0.45\textwidth]{images/high-low}
    \caption{TBA.}
    \label{fig:high_low_issue}
\end{figure}




